The MAPS Algorithm: Fast model-agnostic and distribution-free prediction intervals for supervised learning

A fundamental problem in modern supervised learning is computing reliable conditional prediction intervals in high-dimensional settings: existing methods often rely on restrictive modelling assumptions, do not scale as predictor dimension increases, or only guarantee marginal (population-level) rather than conditional (individual-level) coverage. We introduce the $\textit{lifted predictive model}$ (LPM), a new conditional representation, and propose the MAPS (Model-Agnostic Prediction Sets) algorithm that produces distribution-free conditional prediction intervals and adapts to any trained predictive model. Our procedure is bootstrap-based, scales to high-dimensional inputs and accounts for heteroscedastic errors. We establish the theoretical properties of the LPM, connect prediction accuracy to interval length, and provide sufficient conditions for asymptotic conditional coverage. We evaluate the finite-sample performance of MAPS in a simulation study, and apply our method to simulation-based inference and image classification. In the former, MAPS provides the first approach for debiasing neural Bayes estimators and constructing valid confidence intervals for model parameters given the estimators, at any desired level. In the latter, it provides the first approach that accounts for uncertainty in model calibration and label prediction.

==> jmlr-style-file-master/main_manuscript/class.tex <==
subsection{Adapting MAPS prediction intervals for binary classification}
We generalise MAPS to {\em classification} problems by exploiting the iteratively reweighted least squares (IRLS) algorithm~\citep[Chapter 4.4]{statLearn}. Let $\varphi : \, \mathbb{R} \longrightarrow (0, 1)$ be a link (activation) function that maps a {\em decision boundary}, $\hat{f}: \, \mathbb{R}^d \longrightarrow \mathbb{R}$, to a conditional probability. We assume that the data are generated by the generalised lifted predictive model for a latent response
\begin{equation}\label{eq: logistic LPM}
    Z_o = y_{\beta} (\bx_o) + \frac{Y_o - \varphi_\beta (\bx_o) }{\varphi_{\beta} (\bx_o)  \, \{ 1 - \varphi_{\beta} (\bx_o)\} },
\end{equation}
where $Y_o \, | \, \hat{f} (\bx_o) \sim \operatorname{Bernoulli}[\varphi_{\beta} (\bx_o) ]$ and $\varphi_{\beta} (\bx_o) := \varphi( y_{\beta} (\bx_o) )$, $y_{\beta}$ as in~\eqref{eq: lpm mean-bias definition}. If~\eqref{eq: logistic LPM} is valid, then the negative log-likelihood (deviance loss) is
\begin{equation}\label{eq: lifted deviance}
    \mathcal{L}_{\ell p m} (\calb{\boldsymbol{y}} \, ; \boldsymbol{\beta} ) = - \sum_{\calb{i} = 1}^{\calb{n}} y_{\calb{i}} \operatorname{logit} \{ \varphi( y_{\beta} (\bx_{\calb{i}}) ) \} +
     \log \{ 1 - \varphi( y_{\beta} (\bx_{\calb{i}}) ) \}.
\end{equation}

In view of~\eqref{eq: lifted deviance}, we choose the sigmoid, $\varphi(t) = \exp(t) \, / (1 + \exp(t) )$, as the link function. Let $\mathbf{X} (\hat{f})$ be the $\calb{n} \times 2$ design matrix with ones (intercept) in the first column and decision boundary (logits) entries $\hat{f} (\bx_{\calb{i}})$ in the second column. Then, the Hessian of~\eqref{eq: lifted deviance} is,
\begin{equation*}
    \nabla^2_{\boldsymbol{\beta}} \, \mathcal{L}_{\ell p m} (\calb{\boldsymbol{y}} \, ; \boldsymbol{\beta} ) = \mathbf{X} (\hat{f})^T \mathbf{W} (\varphi_{\beta}) \mathbf{X} (\hat{f}),
\end{equation*}
where $\mathbf{W} (\varphi_{\beta})$ is an $\calb{n} \times \calb{n}$ diagonal matrix with entries $w_{\calb{i}} = \varphi( y_{\beta} (\bx_o) ) \, \{ 1 - \varphi( y_{\beta} (\bx_o) ) \}$.
\begin{algorithm}[H]
\caption{ {\bf IRLS} for lifted binary classification} \label{alg: IRLS for lifted logistic LPM}
    \begin{algorithmic}[1]
        \Require  $(\calb{\mathbf{X}}, \calb{\boldsymbol{y}})$, $\varphi$, $\hat{f}$, $\boldsymbol{\beta}^{(0)}$
        \newline
        {\bf Repeat until convergence} $(t \gets t + 1)$:
        \State $\boldsymbol{z}^{(t)} \gets \mathbf{X} (\hat{f}) \, \boldsymbol{\beta}^{(t - 1)} + \mathbf{W} (\varphi_{\beta})^{-1} \, \left ( \calb{\boldsymbol{y}} - \boldsymbol{\varphi}_{\beta} \right )$
        \State $\boldsymbol{\beta}^{(t)} \gets \underset{\beta}{\operatorname{argmin}} \left \{ (\boldsymbol{z}^{(t)} - \mathbf{X} (\hat{f}) \, \boldsymbol{\beta} )^T \, \mathbf{W} (\varphi_{\beta}) \, (\boldsymbol{z}^{(t)} - \mathbf{X} (\hat{f}) \, \boldsymbol{\beta} ) \right \}$ \Comment{WLS problem}
        \State $\boldsymbol{\varphi}_{\beta} \gets \left \{ \varphi \left ( \beta_0^{(t - 1)} + \beta_1^{(t - 1)} \, \hat{f} (\bx_{\calb{i}}) \right ) \right \}_{\calb{i} = 1}^{\calb{i} = \calb{n}}$
        \State $\mathbf{W}_{\varphi_{\beta}} \gets \operatorname{diag} \left ( \boldsymbol{\varphi}_{\beta} \right )$
    \end{algorithmic}
     $\mathbf{Return:} \hat{\beta}_0, \, \hat{\beta}_1$
\end{algorithm}
Algorithm~\ref{alg: IRLS for lifted logistic LPM} has attractive properties that link its output with a sampling distribution. Using known results for linear logistic regression we obtain a sampling distribution for lifted predictive logits, no matter the distribution of $\hat{f} (\bx_o)$ or of $\boldsymbol{\hat{\beta}}$, nor the dimension of $\bx_o$. This allows us to generalise MAPS to binary classification tasks.
\begin{lemma}\label{lem: sampling classification dist}
    Assume that~\eqref{eq: logistic LPM} is valid, and let $\boldsymbol{\hat{\beta}}$ denote the output of Algorithm~\ref{alg: IRLS for lifted logistic LPM}. Then, $\boldsymbol{\hat{\beta}}$ minimises the loss function in~\eqref{eq: lifted deviance} and 
    \begin{equation}\label{eq: logistic LPM asymp distribution}
        \boldsymbol{\hat{\beta}} \overset{\mathbf{d}}{\longrightarrow} \mathcal{N}_2 \left ( \boldsymbol{\beta}, \, \left ( \mathbf{X} (\hat{f})^T \, \mathbf{W} (\varphi_{\beta}) \, \mathbf{X} (\hat{f}) \right )^{-1} \right ),
    \end{equation}
    where $\boldsymbol{\beta}$ are the unknown parameters of the {\em LPM} in~\eqref{eq: logistic LPM}.
\end{lemma}
\par
The distribution of $Z_o$ is discrete, so its residuals, 
\begin{equation}\label{eq: logit residuals}
    \hat{u}_{\varphi} (\bx_o) = Z_o - \hat{\varphi}_{\beta} (\bx_o),
\end{equation}
where $\hat{\varphi}_{\beta} (\bx_o) = \varphi(\hat{\beta}_0 + \hat{\beta}_1 \, \hat{f} (\bx_o)) $ are lifted predictive logits, also have a discrete distribution, c.f., the continuous residuals in~\eqref{eq: lifted pred error}. This prohibits using a nonparametric density estimator to estimate the distribution of logit residuals in~\eqref{eq: logit residuals}. Lemma~\ref{lem: sampling classification dist} allows us to circumvent this by replacing the density estimator with the known asymptotic distribution for any predictive model. That is, for binary classification tasks we can think of the asymptotic distribution in~\eqref{eq: logistic LPM asymp distribution} as the density estimator $\widehat{P}_{\boldsymbol{\hat{\beta}}}$, and use it for sampling logit residuals and binary responses. First we sample
\begin{equation*}
     \boldsymbol{\beta}_* \sim \mathcal{N}_2 \left ( \boldsymbol{\hat{\beta}}, \, \left ( \mathbf{X} (\hat{f})^T \, \mathbf{W} (\hat{\varphi}_{\beta}) \, \mathbf{X} (\hat{f}) \right )^{-1} \right ),
\end{equation*}
to get a bootstrapped lifted response mean, $\overline{z}_* = \beta_{0, *} + \beta_{1, *} \hat{f} (\calb{\bx})$, and then sample a bootstrap binary response $Y_* \sim \mathrm{Bernoulli} [ \varphi ( \overline{z}_*) ]$, and a lifted latent response
\begin{equation} \label{eq: lifted logit latent response}
    Z_* = \overline{z}_* + \frac{Y_* - \varphi ( \overline{z}_*) }{\varphi ( \overline{z}_*) \{ 1 - \varphi ( \overline{z}_*) \}},
\end{equation}
for computing a bootstrap coefficient estimator
\begin{equation}\label{eq: boostrap logit coeffs solver}
    \boldsymbol{\hat{\beta}}_* = ( \mathbf{X} (\hat{f})^T \, \mathbf{W} (\varphi_{\beta}^*) \, \mathbf{X} (\hat{f}) )^{-1} \mathbf{X} (\hat{f})^T \mathbf{W} (\varphi_{\beta}^*) \boldsymbol{ Z_*}.
\end{equation}
\par
Algorithm~\ref{alg: maps for binary class} bootsraps these steps for estimating the distribution of the predictive logit and its sigmoid, which equals the prediction probability, i.e., $\varphi (\overline{z}_o) = \mathbf{Pr} ( Y_o = 1 \, | \, \hat{f} (\bx_o) )$. This suggests that a prediction interval for $\overline{z}_o$ is a prediction interval for the decision boundary. If for a prediction set, $\widehat{C} (\bx_o)$, we have
\begin{equation*}
    \mathbf{Pr} \left ( \overline{z}_o \in \widehat{C} (\bx_o) \, | \, \hat{f} (\bX_o) = \hat{f} ( \bx_o) \right ) \geq 1 - \alpha,
\end{equation*}
then, since $\varphi$ is {\em monotonic}, we can $\varphi$-transform the quantiles and obtain a prediction interval for the prediction probability,
\begin{equation}\label{eq: maps intervals for binary classification}
    \mathbf{Pr} \left ( p( Y_o = 1 \, | \, \hat{f} (\bx_o) ) \in \varphi \left ( \widehat{C} (\bx_o) \right ) \, | \, \hat{f} (\bX_o) = \hat{f} ( \bx_o) \right ) \geq 1 - \alpha,
\end{equation}
where $\varphi ( \widehat{C} (\bx_o) )$ denotes the intervals we get when $\varphi$-transforming the upper and lower quantiles, i.e., $\varphi ( \widehat{q}_{\alpha} (\overline{z}_o) )$. Note that if~\eqref{eq: logistic LPM} is valid, then we can estimate $\varphi ( \overline{z}_o )$ with $\varphi ( \hat{y}_{\beta} (\bx_o) )$. Combining this with~\eqref{eq: maps intervals for binary classification}, we obtain the MAPS prediction intervals for binary classification at the $(1 - \alpha) \times 100\%$ confidence level,
\begin{equation} \label{eq: MAPS binary class}
    \widehat{C}_{\operatorname{maps} } (\bx_o; \, \varphi ) = \left [ \varphi (\hat{y}_{\beta} (\boldsymbol{x}_{o} ) + \widehat{q}_{\alpha / 2} (\hat{r}_o) ), \, \varphi (\hat{y}_{\beta} (\boldsymbol{x}_{o} ) + \widehat{q}_{1 - \alpha / 2} (\hat{r}_o) ) \right ]
\end{equation}
where $\hat{r}_o := \hat{y}_{\beta} (\boldsymbol{x}_{o} ) - \hat{z}_o$ is the random difference between $\hat{y}_{\beta} (\boldsymbol{x}_{o} )$ and bootstrap estimates for $\overline{z}_o = y_{\beta} (\boldsymbol{x}_{o} )$, and $\widehat{q}_{\alpha / 2} (\hat{r}_o )$ and $ \widehat{q}_{1 - \alpha / 2} (\hat{r}_o )$ are computed using Algorithms~\ref{alg: IRLS for lifted logistic LPM} and~\ref{alg: maps for binary class}.

\begin{algorithm}
\caption{ {\bf MAPS} for binary classification}\label{alg: maps for binary class}
    \begin{algorithmic}[1]
        \Require  $(\calb{\mathbf{X}}, \calb{\boldsymbol{y}})$, $\boldsymbol{x}_o$, $\hat{f}$, miscoverage level $\alpha$ 
        \State $(\hat{\beta}_0, \, \hat{\beta}_1 ) = \underset{\beta_0, \, \beta_1}{\mathrm{argmin}} \left \{ \mathcal{L}_{\ell p m} \left ( \calb{\boldsymbol{y}}, \, \hat{f} \right ) \right \}$ \Comment{Generalised LPM in~\eqref{eq: lifted deviance}}
        
        % \State $\hat{u}  (\bx_{\calb{i}}) = [y_{\calb{i}} - \varphi( \hat{y}_{\beta} (\bx_{\calb{i}}) )] / \, [\varphi( \hat{y}_{\beta} (\bx_{\calb{i}}) ) \, \{ 1 - \varphi( \hat{y}_{\beta} (\bx_{\calb{i}}) ) \}]$ \Comment{Bernoulli errors}

        \State $\hat{y}_{\beta} (\bx_{\calb{i}}) = \hat{\beta}_0 + \hat{\beta}_1 \, \hat{f} (\bx_{\calb{i}} )$
        
        %\State $V_{\calb{i}} = \widehat{P}_{\hat{y}}  ( \hat{y}_{\beta} (\bx_{\calb{i}}) \, | \,  \hat{f} (\bx_{\calb{i}}) )$ 
        \For{$b = 1$ to $b = B$}
            %\State $\boldsymbol{V}^{(b)} \sim \{ V_{\calb{1}}, \dots, V_{\calb{n}} \}$ \Comment{Sample pivots for $\calb{\overline{z}}$}
            \State $\boldsymbol{\beta}^{(b)} \sim \mathcal{N}_2 \left ( \boldsymbol{\hat{\beta}}, \, \left ( \mathbf{X} (\hat{f})^T \, \mathbf{W} (\hat{\varphi}_{\beta}) \, \mathbf{X} (\hat{f}) \right )^{-1} \right )$

            \State $\overline{z}^{(b)}_{\calb{i}} = \beta_{0}^{(b)} + \beta_{1}^{(b)} \hat{f} (\bx_{\calb{i}})$

            \State $Y_{\calb{i}}^{(b)} \sim \operatorname{Bernoulli} \left [ \varphi \left (\overline{z}^{(b)}_{\calb{i}} \right ) \right ]$

            \State $Z^{(b)}_{\calb{i}} = \overline{z}^{(b)}_{\calb{i}} + (Y_{\calb{i}}^{(b)} - \varphi(\overline{z}^{(b)}_{\calb{i}}) ) / \{ \varphi (\overline{z}^{(b)}_{\calb{i}}) ( 1 - \varphi(\overline{z}^{(b)}_{\calb{i}}) ) \}$ \Comment{ Bootstrap responses in~\eqref{eq: lifted logit latent response}}

            \State $ \boldsymbol{\hat{\beta}}^{(b)} = ( \mathbf{X} (\hat{f})^T \, \mathbf{W} (\varphi_{\beta}^{(b)}) \, \mathbf{X} (\hat{f}) )^{-1} \mathbf{X} (\hat{f})^T \mathbf{W} (\varphi_{\beta}^{(b)}) \boldsymbol{ Z}^{(b)}$

            \State $\hat{z}^{(b)}_o = \hat{\beta}_0^{(b)} + \hat{\beta}_1^{(b)} \, \hat{f} (\bx_o )$
        
            \State $\hat{r}_o^{(b)} = \hat{y}_{\beta} (\boldsymbol{x}_{o} ) - \hat{z}^{(b)}_o $ \Comment{Bootstrap prediction logit error}
            
        \EndFor
        
        \State Compute $\widehat{q}_{\alpha / 2} (\hat{r}_o ), \, \widehat{q}_{1 - \alpha / 2} (\hat{r}_o )$ \Comment{Empirical quantiles of $\{ \hat{r}^{(b)} \} $ }
        
    \end{algorithmic}
     $\mathbf{Return:} \, \hat{y}_{\beta} (\boldsymbol{x}_{o} ), \, \widehat{q}_{\alpha / 2} (\hat{r}_o ), \, \widehat{q}_{1 - \alpha / 2} (\hat{r}_o )$
\end{algorithm}

Remark~\ref{rem: attractive logit} shows some of the sigmoid's attractive properties. This choice is popular in the classification literature and facilitates implementing Algorithm~\ref{alg: maps for binary class}. Further, $y_{\beta}$ can be easily modified, e.g., if we constrain $\beta_0 = 0$ and set $\beta_1 = 1 / T$ for $T > 0$, then $\varphi( y_{\beta} (\bx_o) )$ mimics {\em temperature scaling}~\citep{prob_calib_temp_scaling}. Interestingly, the lifted prediction probabilities, $\varphi( \hat{y}_{\beta} (\bx_o) )$, are related, and can be made equal, to the ones \cite{Platt1999} originally proposed for support vector classifiers, albeit obtained with different models and motivations, since the latter are not used for computing prediction intervals nor model comparison, and sometimes are fitted using scores rather than responses. Due to space constraints, we do not develop extensions to alternate link functions or methods for estimating the link function, e.g., isotonic regression, nor explore connections to discriminant analysis, scores and separation margins, we leave these for future work.

\begin{remark}\label{rem: attractive logit}
    The decision boundary for an out-of-sample point is $\{ \bx_o : \, \hat{y}_{\beta} (\bx_o ) = 0 \}$, which adjusts the decision boundary given by the predictive model $\hat{f}$. Further, by setting the partial derivatives of~\eqref{eq: lifted deviance} to zero we see that $\calb{\overline{y}} = (1 / \, \calb{n} ) \, \sum_{\calb{i} = 1}^{\calb{n}} \varphi ( \hat{y}_{\beta} (\bx_{\calb{i}} ) )$, i.e., the expected number of successes matches the average probability of success, and if $\beta_1 = 0$, then the decision boundary of $Y_o$ does not depend on $\hat{f} (\bx_o)$, i.e, $\varphi ( \hat{y}_{\beta} (\bx_o ) ) = \calb{\overline{y}}$ for all $\bx_o$. 
\end{remark}

==> jmlr-style-file-master/main_manuscript/lpm_heory_and_pred_intervals.tex <==
\section{Prediction intervals and the LPM}
\label{sec: pred intervasla and LPM}
% We remind the reader that our main interest is computing valid, non-trivial and model-agnostic prediction intervals for an unknown response value $y_o$ based on the (realised) pointwise prediction $\hat{f} (\boldsymbol{x}_o)$, i.e., the prediction intervals are valid confidence intervals without constraining the regression family nor fixing a learning algorithm for obtaining $\hat{f}$. We begin by analysing the problem in an ideal setting. 
Recall that the data are generated by~\eqref{eq: regression error} and isolate the out-of-sample error term
\begin{equation} \label{eq: regression error term}
    \epsilon_o := Y_o - f(\boldsymbol{x}_o),
\end{equation}
where we assume that $ \epsilon_o \, | \, f(\boldsymbol{X}_o) = f(\boldsymbol{x}_o) \sim P_{\epsilon}$. Computing a prediction interval centred at $f(\boldsymbol{x}_o)$ is straightforward if we have access to $f$ and the quantiles $q_{\alpha} \big ( \epsilon_o \big ) = P_{\epsilon}^{-1} \big (\alpha \, | \, f(\boldsymbol{x}_o) \big )$ of the regression error distribution, i.e., for $\alpha \in (0, 1)$ we have that $\mathbf{Pr} \big \{ \epsilon_o \leq q_{\alpha} \big ( f(\boldsymbol{x}_o) \big )  \big \} = \alpha$. In this ideal case, the natural prediction interval at the $(1 - \alpha) \times 100\%$ confidence level is 
\begin{equation} \label{eq: ideal oracle confidence region}
    C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right ) := \big [ f(\boldsymbol{x}_o) + q_{\alpha / 2} ( \epsilon_o ), \, f(\boldsymbol{x}_o) + q_{1 - \alpha / 2} ( \epsilon_o ) \big ],
\end{equation}
where the quantiles switch places if $\alpha > 1/2$. Thus, for all possible $\boldsymbol{x}_o$ we have that
\begin{equation*}
    \mathbf{Pr} \big ( Y_o \in  C_{\mathrm{ideal}} (\boldsymbol{x}_o)  \, | \, \boldsymbol{X}_o = \boldsymbol{x}_o  \big ) = 1 - \alpha.
\end{equation*}
\par
Note that the quantiles are a function of $\alpha$ and $f (\boldsymbol{x}_o)$, i.e., the length of the conditional prediction interval
\begin{equation*}
     \lambda_{\mathrm{Leb}} \left( C_{\mathrm{ideal}} (\boldsymbol{x}_o) \right) = \left | \, q_{1 - \alpha / 2} \big (\epsilon_o \big ) - q_{\alpha / 2} \big ( \epsilon_o \big ) \right |,
\end{equation*}
where $\lambda_{\mathrm{Leb}}$ is the Lebesgue measure (interval length), depends on its miscoverage level, $\alpha$, and centre, $f (\bx_o) $. If we assume that the out-of-sample regression errors in~\eqref{eq: regression error} are generated by an absolutely continuous distribution, then the optimal (tightest) prediction interval is $ C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right )$; see~\cite{dcp} for an earlier equivalent version based on response quantiles, rather than on the regression function and error quantiles.
\begin{proposition}\label{prop: ideal optimal interval}
    The interval $ C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right )$ in~\eqref{eq: ideal oracle confidence region} solves the optimisation problem
    \begin{equation}\label{eq: optmial pred interval optimisation}
         C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right ) =\underset{C ( \bx_o) }{\operatorname{argmin}} \left \{ \lambda_{\mathrm{Leb}} \left (   C \left ( \boldsymbol{x}_o \right ) \right ) \right \} \, \, \, s.t. \, \, \, \mathbf{Pr} \big ( Y_o \in  C (\boldsymbol{x}_o)  \, | \, \boldsymbol{X}_o = \boldsymbol{x}_o  \big ) \geq 1 - \alpha,
    \end{equation}
    for all $\alpha \in (0, 1)$, where $\bx_o \in \mathcal{X}$ and $C ( \bx_o)  \subset \mathbb{R}$ is a prediction interval.
\end{proposition}
\par
Unfortunately, neither the regression function $f$ nor the error distribution $P_{\epsilon}$ is known in practice. To address this, we extend the ideal prediction interval construction to any predictive model $\hat{f}$ by centring the prediction interval at $\hat{f} (\boldsymbol{x}_o)$. The residuals associated with model $\hat{f}$ are
\begin{equation} \label{eq: prediction error}
    \hat{\epsilon}_o := Y_o - \hat{f} (\boldsymbol{x}_o ), 
\end{equation}
given $\hat{f}(\boldsymbol{X}_o) = \hat{f} (\boldsymbol{x}_o)$. These can be decomposed into regression and model estimation errors, i.e., $\hat{\epsilon}_o = \epsilon_o + (f (\bx_o) - \hat{f} (\bx_o) )$. If we had access to the quantiles of $\hat{\epsilon}_o$, then we could compute the oracle prediction intervals
% That is, the prediction error is the random difference between the observed response and model prediction, and it can be decomposed into regression and model estimation errors, i.e., $\hat{\epsilon}_o = \epsilon_o + (f (\bx_o) - \hat{f} (\bx_o) )$. Even when the true noise distribution $P_\epsilon$ is Gaussian, the induced distribution $P_{\hat{\epsilon}}$ of $\hat{\epsilon}$ need not to be Gaussian; see the experiments in Section [TO ADD]. If we had access to the quantiles of $\hat{\epsilon}_o$, then we could compute the oracle prediction intervals
\begin{equation}\label{eq: oracle pred interval}
     \widehat{C}_{\mathrm{oracle}} \left ( \boldsymbol{x}_o \right ) := \big [ \hat{f} (\boldsymbol{x}_o) + q_{\alpha / 2} \big ( \hat{\epsilon}_o ) \big ), \, \hat{f} (\boldsymbol{x}_o) + q_{1 - \alpha / 2} \big (\hat{\epsilon}_o \big ) \big ],
\end{equation}
which guarantee coverage at the $(1 - \alpha) \times 100\%$ level. 
\begin{remark}
    Interestingly, even when the true noise distribution $P_\epsilon$ is Gaussian, the induced distribution $P_{\hat{\epsilon}}$ of $\hat{\epsilon}$ need not to be Gaussian; see the experiments in Section [TO ADD].
\end{remark}
\par
We can measure the distance between $ C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right )$ and $\widehat{C}_{\mathrm{oracle}} \left ( \boldsymbol{x}_o \right )$ as the length of their symmetric difference, $ \lambda_{\mathrm{Leb}} ( C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right ) \Delta \widehat{C}_{\mathrm{oracle}} \left ( \boldsymbol{x}_o \right ) )$, which for intervals equals
\begin{multline*}
    \big | \{ \hat{f} (\boldsymbol{x}_o) - f (\boldsymbol{x}_o) \} + \{ q_{1 - \alpha / 2} (\hat{\epsilon}_o ) - q_{1 - \alpha / 2} (\epsilon_o ) \} \big | + \\
    \big | \{ \hat{f} (\boldsymbol{x}_o) - f (\boldsymbol{x}_o) \} + \{ q_{\alpha / 2} (\hat{\epsilon}_o ) - q_{\alpha/2}(\epsilon_o ) \} \big |,
\end{multline*}
\par
whence, estimating the regression function with precision {\em decreases} the distance between $ C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right )$ and $\widehat{C}_{\mathrm{oracle}} \left ( \boldsymbol{x}_o \right )$. That is, if $\hat{f} (\boldsymbol{x}_o) \approx f (\boldsymbol{x}_o)$, then $q_{\alpha} (\hat{\epsilon}_o ) \approx q_{\alpha} (\epsilon_o )$, which follows from continuity of the cumulative distribution and quantile functions. Put another way, the more accurate a model is, the more $\epsilon_o$ and $\hat{\epsilon}_o$ will be similar random variables, i.e., if $\hat{f} \approx f$, then $P_{\epsilon} \approx P_{\hat{\epsilon}}$. Recall the little-$o$ notation for convergence in probability, i.e., if $\mathbf{Pr} ( \| \hat{f} - f \|_{\infty} \leq \delta ) \to 1$ for all $\delta > 0$ as $n_{\mathrm{train}} \to +\infty$, we write $ \| \hat{f} - f \|_{\infty} = o_{\mathbf{Pr}} (1)$, and say that $\hat{f}$ is a supremum-norm consistent estimator of $f$. Lemma~\ref{lem: oracle and ideal coverage} highlights that if $\hat{f}$ is accurate, then $\widehat{C}_{\mathrm{oracle}} ( \boldsymbol{x}_o )$ is asymptotically optimal. Hence, model estimation plays an important role in the construction of prediction intervals.
\begin{lemma}\label{lem: oracle and ideal coverage}
    Assume that $\| \hat{f} - f \|_{\infty} = o_{\mathbf{Pr}} (1)$ and that $P_{\epsilon}$ is continuous for all $\bx_o$. Then, we have that $P_{\hat{\epsilon}} (t) \to P_{\epsilon} (t)$ for all $t \in \mathbb{R}$ and
    \begin{equation}\label{eq: oracle and ideal converge}
         \lambda_{\mathrm{Leb}} \left ( C_{\mathrm{ideal}} \left ( \boldsymbol{x}_o \right ) \Delta \widehat{C}_{\mathrm{oracle}} \left ( \boldsymbol{x}_o \right ) \right ) \overset{\mathbf{Pr}}{\longrightarrow} 0.
    \end{equation}
\end{lemma}
\par
% Adapting Proposition~\ref{lem: oracle and ideal coverage} for $\hat{\epsilon}$ in~\eqref{eq: prediction error} shows that for any $\hat{f}$, $\widehat{C}_{\mathrm{oracle}} ( \boldsymbol{x}_o )$ is the best we can do, i.e., it solves~\eqref{eq: optmial pred interval optimisation} constrained to prediction intervals centred at $\hat{f} (\bx_o)$.
\begin{remark}\label{rem: require accurate centre and quantiles}
   {\em Lemma~\ref{lem: oracle and ideal coverage}},~\eqref{eq: prediction error} and~\eqref{eq: oracle pred interval} elucidate that we require accurate estimates of the conditional distribution of the residuals $\hat{\epsilon}_o$--\underline{not of the regression errors $\epsilon$}--to enable uncertainty attain conditional coverage guarantees. That is, we need both an accurate estimate of the centre and precise estimates of the resulting residual quantiles.
\end{remark}
\par
Remark~\ref{rem: require accurate centre and quantiles} tells us that we need both an accurate estimate of the centre and precise estimates of the resulting residual quantiles. Note that balancing the MSPE~\eqref{eq: mspe definition} should produce more accurate predictive models, and residuals that approximate the error in~\eqref{eq: regression error term}. This, would allow us to estimate the distribution and quantiles of the resulting residuals, which will be referred to as lifted residuals; see Section~\ref{subsubsec: real_valued_case}. We use MAPS to estimate these quantiles, which can then be substituted into the prediction interval construction in~\eqref{eq: oracle pred interval}, resulting in theoretically grounded, model-agnostic and distribution-free conditional prediction intervals.
%
\subsection{LPM with noise in the classic setting}
In the classic setting we assume the LPM given by
\begin{equation} \label{eq: classic setting lpm}
    \calb{Y} = y_{\beta} (\calb{\bx}) + u, 
\end{equation}
where $y_{\beta} (\calb{\bx}) := \beta_0 + \beta_1 \hat{f} (\calb{\bx})$, 
%$\var ( \calb{Y} ) = \var(f) + \sigma_{\epsilon}^2$, $\var(f) = \int \{f(\bx) - \mu(f) \}^2 dP_{\bx}$, $\mu(f) := \int f(\bx) dP_{\bx}$,
and the error linked to $\hat{f}$ is Gaussian, i.e., $u \sim \mathcal{N} (0, \sigma_{u}^2)$; see~\cite{salnikov2024liftedcoefficientdeterminationfast} for an earlier version of~\eqref{eq: classic setting lpm}. 
% \begin{remark}
    % The {\em LPM} given by~\eqref{eq: classic setting lpm} can be derived from a bivariate Gaussian assumption that links the correlation between calibration observations and model predictions;
%     Formally, it is derived from the conditional mean of $\calb{Y} \, | \, \hat{f} (\calb{\bx})$ if we assume that
%     \begin{equation*}
%     \begin{Bmatrix} 
%     \calb{Y} \\ \hat{f} (\calb{\bx}) 
%     \end{Bmatrix} \sim \mathcal{N}_2 \bigg [ \begin{Bmatrix} f(\calb{\bx}) \\ \overline{f} (\calb{\bx}) \end{Bmatrix},
%     \begin{pmatrix} \mathrm{var} (\calb{Y}) & \mathrm{cov} \{ \calb{Y}, \overline{f} (\calb{\bx}) \} \\ \mathrm{cov} \{ \calb{Y}, \overline{f} (\calb{\bx}) \} & \mathrm{var} (\overline{f}) \end{pmatrix} \bigg ].
% \end{equation*}
% \end{remark}
Note that~\eqref{eq: classic setting lpm} connects data generated by~\eqref{eq: regression error} with model predictions $\hat{f} (\calb{\bx})$ via a known joint distribution function. We stress that the random errors in~\eqref{eq: classic setting lpm} are {\em different} from the ones in~\eqref{eq: regression error}, i.e., $P_{u}$ is not the same as $P_{\epsilon}$, e.g., if~\eqref{eq: classic setting lpm} is valid, then $\var (u) = ( 1 - \rho^2) \{\var(f) + \sigma_{\epsilon}^2 \}$, which is equal to $\sigma_{\epsilon}^2$ if the regression function is constant, $f \equiv C$, or if $\beta_0 = 0$, $\beta_1 = 1$ and $\hat{f} \equiv f$ (in probability). Hence, we can derive a known prediction error distribution within the classic setting of linear regression with Gaussian errors. We estimate the unknown bias, $\beta_0$, and precision, $\beta_1$, coefficients in~\eqref{eq: classic setting lpm} by least-squares, and express the estimators in an alternative form, which highlights the interval's dependence on the correlation between model predictions and calibration response values.
The prediction interval, $\widehat{C}_{\ell pm} (\bx_o)$, is 
\begin{equation} \label{eq: b0 lpm prediction interval}
     \hat{y}_{\beta} (\bx_o) \pm \left \{ \left [1 + 1 / (n_{\mathrm{cal}} - 2) \right ] \left [ 1 - \calb{R^2} (\hat{f}) \right ] s_{\calb{\boldsymbol{y}}}^2 \left [ 1 + \widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) \right ] \right \}^{ 1 / 2 } t_{(n_{\mathrm{cal}} - 2), 1 - \alpha / 2},
\end{equation}
where $\hat{y}_{\beta} (\bx_o) := \hat{\beta}_0 + \hat{\beta}_1 \, \hat{f} (\x_o )$ are lifted predictions, $ \overline{\mu}_{\hat{f}} := ( 1 / \calb{n}) \, \sum_{\calb{i} = 1}^{\calb{n}} \hat{f} (\bx_{\calb{i}})$,
$$\widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) := \frac{1}{ n_{\mathrm{cal}} } + \frac{( \hat{f} (\bx_o) - \overline{\mu}_{\hat{f}})^2 }{ \sum_{i = 1}^{n_{\mathrm{cal}}} ( \hat{f} ( \bx_{\calb{i}}) -  \overline{\mu}_{\hat{f}})^2  }, $$
%% \begin{align*}
%     &\overline{y}_{\mathrm{cal}} = 1 / n_{\mathrm{cal}}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} y_{i_{\mathrm{cal}}}, \, \, \, \, \, \, \, \, \, \, \, \,  s_{y_{\mathrm{cal}}}^2 = (n_{\mathrm{cal}} - 1)^{-1}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} (y_{i_{\mathrm{cal}}} - \overline{y}_{\mathrm{cal}} )^2, \\
%     &\hat{\mu}_{\mathrm{cal}} = 1 / n_{\mathrm{cal}}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} \hat{f} (\boldsymbol{x}_{i_{\mathrm{cal}}}), \, \, \, \, \, \,
%     s_{\hat{f}}^2 = (n_{\mathrm{cal}} - 1)^{-1}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} \{ \hat{f} (\boldsymbol{x}_{i_{\mathrm{cal}}}) - \hat{\mu}_{\mathrm{cal}} \}^2,
% \end{align*}
% are sample mean and standard deviation statistics for response and model predictions in the calibration set, and
and $\calb{R} (\hat{f})$
    %$= \left [ \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} (y_{i_{\mathrm{cal}}} - \overline{y}_{\mathrm{cal}})  \{ \hat{f} (\boldsymbol{x}_{i_{\mathrm{cal}}}) - \hat{\mu}_{\mathrm{cal}} \} \right ] / ( s_{y_{\mathrm{cal}}} \, s_{\hat{f}} )$
is the correlation coefficient between $\calb{\boldsymbol{y}}$ and $\{ \hat{f} (\boldsymbol{x}_{1_{\mathrm{cal}}}), \dots, \hat{f} (\boldsymbol{x}_{n_{\mathrm{cal}}}) \}$.
\par
The prediction interval $\widehat{C}_{\ell pm} (\bx_o)$ is model-agnostic at the $(1 - \alpha) \times 100\%$ confidence level, i.e., it is a valid non-trivial prediction interval for any model $\hat{f}$. Further, it suggests comparing predictive models using correlation values, since its length {\em decreases} the closer $R_{\mathrm{cal}}^2 (\hat{f})$ is to one, and that the MSPE of lifted predictions is smaller than the one of model predictions $\hat{f} (\calb{\bx})$.
%, i.e., $\sum_{\calb{i} = 1}^{\calb{n}} (y_{\calb{i}} - \hat{y}_{\beta} (\bx_{\calb{i}}) )^2 \leq \sum_{\calb{i} = 1}^{\calb{n}} (y_{\calb{i}} - \hat{f} (\bx_{\calb{i}}) )^2$. 
Theorem~\ref{th: t student interval} makes these statements precise.
\begin{theorem} \label{th: t student interval}
    Assume that~\eqref{eq: classic setting lpm} is valid. Then, given $\hat{f} (\boldsymbol{x}_o)$ and $\{ \hat{f} (\boldsymbol{x}_{1_{\mathrm{cal}}}), \dots, \hat{f} (\boldsymbol{x}_{n_{\mathrm{cal}}}) \}$, for all $\alpha \in (0, 1)$ we have that
    % \begin{equation} \label{eq: t-student distribution}
    %     U_o / \big \{ a^2 \big(1 - R^2_{\mathrm{cal}} (\hat{f}) \big) s_{y_{\mathrm{cal}}}^2 \hat{\eta} (\boldsymbol{x}_o ) \big \}^{ 1 / 2 } \sim t (n_{\mathrm{cal}} - 2),
    % \end{equation}
    % where $t (n_{\mathrm{cal}} - 2)$ is Student's t-distribution with $(n_{\mathrm{cal}} - 2)$ degrees of freedom. Thus, for $\alpha \in (0, 1)$ we have that
            \begin{equation} \label{eq: point estimator concentration}
                  \mathbf{Pr} \big ( Y_o \in \widehat{C}_{\ell pm} (\bx_o) \, | \, \bX_o = \bx_o \big ) = 1 - \alpha.
            \end{equation}
    Further, for homoscedastic errors, not necessarily Gaussian, the {\em MSPE} can be bounded as
    \begin{equation}
        \operatorname{MSPE} [ f (\bx_o)] \leq \operatorname{MSPE} [y_{\beta} (\bx_o)] \leq \operatorname{MSPE} [\hat{f} (\bx_o)],
    \end{equation}
    and we have that
    \begin{equation*}
        \operatorname{MSPE} [\hat{y}_{\beta} (\bx_o)] = \operatorname{MSPE} [y_{\beta} (\bx_o)] + o( 1 / \, \calb{n}).
    \end{equation*}
    % \begin{multline} \label{eq: mspe lower bound}
    %         \sigma_{\epsilon}^2 + \sigma_u^2 \mathbb{E} \big[ \widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) \big] \leq \operatorname{MSPE} [\hat{y}_{\beta} (\bx_o)]
    %         \leq \sigma_{\epsilon}^2 + \sigma_u^2 \mathbb{E} \big[ \widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) \big] \\
    %        + 2 \left ( \beta_1^2 \, \operatorname{MSPE} [\hat{f} (\bx_o)] + \{ \beta_0 + (\beta_1 - 1) f (\bx_o) \}^2 \right ).
    % \end{multline}
\end{theorem}
\par
Theorem~\ref{th: t student interval} allows us to compute fast model-agnostic conditional prediction intervals with valid finite sample coverage, albeit in the classic setting~\eqref{eq: classic setting lpm}. To the best of our knowledge, there are no other closed-form solution prediction intervals with these properties. Further, if $\hat{f}$ is consistent ($\| \hat{f} - f \|_{\infty} = o_{\mathbf{Pr}} (1)$), then $\hat{y}_{\beta}$ is also consistent, $| \hat{y}_{\beta} (\bx_o) - \hat{f} (\bx_o) | = o_{\mathbf{Pr}} (1)$ and $\widehat{C}_{\ell pm} (\bx_o)$ converges in probability to $C_{\mathrm{ideal}} (\bx_o)$. MAPS generalises $\widehat{C}_{\ell pm} (\bx_o)$ to the distribution-free setting.




%The bounds in~\eqref{eq: mspe lower bound} are valid, and~\eqref{eq: point estimator concentration} is asymptotically valid, for any error distribution $P_u$ as long as the errors are homoscedastic, as in~\eqref{eq: additive errors}. Note that we can think of $\hat{\beta}_0$ as the average bias correction, and of $\hat{\beta}_1$ as $R_{\mathrm{cal}} (\hat{f})$ adjusted by the ratio $s_{y_{\mathrm{cal}}} / s_{\hat{f}}$, which is related to the {\em signal-to-noise} ratio $\mathrm{var} (f) / \sigma_{\epsilon}^2$. Hence, the LPM is a useful tool for comparing, evaluating and improving predictive models. Corollary~\ref{cor: consistent model properties} makes these statements precise.
% \begin{corollary} \label{cor: consistent model properties}
%      Assume that $\| \hat{f} - f \|_{\infty} = o_{\mathbf{Pr}} (1)$. Then, as $n_{\mathrm{train}} \to +\infty$ we have that
%      $$
%         \rho \rightarrow \mathrm{sd} (f) / \{ \mathrm{var} (f) + \sigma^2_{\epsilon} \}^{1 / 2}, \enspace \beta_1 \rightarrow 1 \textit{ and } \, \beta_0 \rightarrow 0,
%     $$ 
%     where $\rho \in [-1, 1]$ is the population correlation coefficient of $\calb{Y}$ and $\hat{f} (\calb{\bX})$. Further, as $\calb{n} \to +\infty$ we have that 
%     %$
%     %    \operatorname{MSPE} [\hat{y}_{\beta} (\bx_o)] = \sigma_{\epsilon}^2 + O(1 / \calb{n})$, 
%     $\| \hat{y}_{\beta} - f \|_{\infty} = o_{\mathbf{Pr}} (1)$, and 
%         $$\lambda_{\mathrm{Leb}} \left ( \widehat{C}_{\ell pm} (\bx_o) \Delta  C_{\mathrm{ideal}} (\bx_o) \right ) = o_{\mathbf{Pr}} (1).$$
% \end{corollary}
%The results in Corollary~\ref{cor: consistent model properties} are still valid for homoscedastic errors with a finite variance. Further, we can define a test based on the statistics in~\eqref{eq: b0 lpm prediction interval} for data generated by~\eqref{eq: additive errors}. We will use the results in Lemma~\ref{lem: homos errors sampling}.
%\begin{lemma} \label{lem: homos errors sampling}
%    Assume that the training and calibration sets are generated by~\eqref{eq: additive errors}, the {\em LPM} in~\eqref{eq: lpm mean-bias definition} is valid for calibration and out-of-sample data, and we estimate the bias and precision parameters by least-squares as in~\eqref{eq: b0 lpm prediction interval}, and the errors $u_{\mathrm{cal}}$, not necessarily Gaussian, satisfy $\mathbb{E}(u) = 0$ and $\mathrm{var} (u_) = \sigma^2_{u} < +\infty$. Then, given $\{ \hat{f} (\boldsymbol{x}_{1_{\mathrm{cal}}} ), \dots,\hat{f} (\boldsymbol{x}_{n_{\mathrm{cal}}} ) \}$, as $\calb{n} \to +\infty$, we have that
 %   \begin{equation*}
 %       \sqrt{n_{\mathrm{cal}}} (\hat{\beta}_0 - \beta_0, \hat{\beta}_1 - \beta_1 ) \overset{\boldsymbol{\mathrm{d}}}{\longrightarrow} \mathcal{N}_2 ( 0, \sigma^2_{u} \, \mathbf{\Hat{\Sigma}} ),
 %   \end{equation*}
 %   where $\mathbf{\Hat{\Sigma}} \propto (\mathbf{Z}^T \mathbf{Z})^{-1}$, and $\mathbf{Z} := [\boldsymbol{1}, \{ \hat{f} (\boldsymbol{x}_{i_{\mathrm{cal}}} ) \} ]$ is the $n_{\mathrm{cal}} \times 2$ design matrix corresponding to model \eqref{eq: lpm mean-bias definition}. Let $\hat{\sigma}^2_u := 1 / (n_{\mathrm{cal}} - 2) \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}}  [ y_{i_{\mathrm{cal}}} - \hat{y} (\boldsymbol{x}_{i_{\mathrm{cal}}} ) ]^2$, i.e., the calibration set mean residual sum of squares. Then, we have that
 %   \begin{equation*}
 %       \big \{ (n_{\mathrm{cal}} - 2)^{1 / 2} / \hat{\sigma}_u \big \} \mathbf{\Hat{\Sigma}}^{1/2} (\boldsymbol{\hat{\beta}} - \boldsymbol{\beta}) \overset{\boldsymbol{\mathrm{d}}}{\longrightarrow} t_{2} (n_{\mathrm{cal}} - 2),
 %   \end{equation*}
 %   where $t_{2} (n_{\mathrm{cal}} - 2)$ is the standard (i.e., zero-mean, covariance $\mathbf{I_2}$) bivariate Student's t-distribution with $(n_{\mathrm{cal}} - 2)$ degrees of freedom.
%\end{lemma}
%By Lemma~\ref{lem: homos errors sampling}, $\hat{\beta}_0$ and $\hat{\beta}_1$ are asymptotically normal and consistent estimators of $\beta_0$ and $\beta_1$. Using $\boldsymbol{\beta} = (\beta_0, \beta_1)$, we test if $\hat{f}$ is a consistent estimator of $f$ by testing the null hypothesis $H_0: \, \beta_0 = 0$ and $\beta_1 = 1$. Let $\alpha \in (0, 1)$ and define the critical region 
%$$\mathcal{C}_{H_0} ( T_{\alpha} ) := \big \{ (\boldsymbol{y}_{\mathrm{cal}}, \hat{f} ) : \max ( | \hat{\beta}_0|, \, |\hat{\beta}_1 - 1| ) > T_\alpha \big \},$$ 
%where $T_{\alpha} > 0$ is the corresponding quantile (e.g., $\ell_{\infty}$-norm radius) of the standard bivariate Student's $t$-distribution with $(n_{\mathrm{cal}} - 2)$ degrees of freedom; see \cite{muitvariate_t_dist} for a review of this distribution. By Lemma~\ref{lem: homos errors sampling}, $\mathcal{C}_{H_0} ( T_{\alpha} )$ is a valid critical region at the $\alpha \times 100\%$ significance level, 
%\begin{equation*}
%    \mathbf{Pr} \left ( \boldsymbol{\beta} \in \mathcal{C}_{H_0} ( T_{\alpha} ) \, | \, H_0 \right ) = \alpha.
%\end{equation*}
% \subsection{Beyond the classic setting}
% Homoscedastic Gaussian errors and a constant bias function could be considered stringent assumptions. We relax distributional assumptions and derive the MAPS algorithm in Section~\ref{sec: maps}. B



==> jmlr-style-file-master/main_manuscript/tables/Table2.tex <==
    \begin{tabular}{lrrrrr}
     $\mathbf{\ntrain, \, \calb{n}}$ & \small\bf{MSPE}$(\mathbf{\hat{f}})$ & \small\bf{MSPE}$(\mathbf{\hat{y}_{\psi}})$ & \small\bf{MSPE Diff} & \small\bf{MAE}$( 0.95, \, \widehat{p}(\x_o) )$ & \small\bf{Length}\\
     \hline\\
    &\multicolumn{5}{r}{{\small\bf Results for SVM:} $\hat{f}_\textrm{SVM}$}\\
    \cline{2-6}\\
    \small 1,000 & \small 15.1 & \small 14.4 & \small $4.3\%$ & \small $4.5\%$ & \small 16.0 \\
    \small 2,500 & \small 10.2 & \small 7.8 & \small $26.3\%$ & \small $3.2\%$ & \small 11.0 \\
    \small 5,000 & \small 6.1 & \small 4.9 & \small $19.7\%$ & \small $1.7\%$ & \small 8.5 \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    \hline\\
    &\multicolumn{5}{r}{{\small\bf Results for GAM:} $\hat{f}_\textrm{GAM}$}\\
    \cline{2-6}\\
    \small 1,000 & \small 0.4 & \small 0.4 & \small $0.0\%$ & \small $1.8\%$ & \small 2.5 \\
    \small 2,500 & \small 0.4 & \small 0.4 & \small $0.0\%$ & \small $0.6\%$ & \small 2.6 \\
    \small 5,000 & \small 0.4 & \small 0.4 & \small $0.0\%$ & \small $0.4\%$ & \small 2.6\\
    \hline\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    &\multicolumn{5}{r}{{\small\bf Results for RF:} $\hat{f}_\textrm{RF}$}\\
    \cline{2-6}\\
    \small 1,000 & \small 1.5 & \small 1.5 & $0.6\%$ & $1.0\%$ & \small 5.0 \\
    \small 2,500 & \small 1.2 & \small 1.2 & \small $1.1\%$ & \small $0.6\%$ & \small 4.3 \\
    \small 5,000 & \small 0.9 & \small 0.8 & \small $0.5\%$ & \small $0.8\%$ & \small 3.9 \\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}

==> jmlr-style-file-master/supplementary_material/classical_setup.tex <==
\subsection{Additive errors and pivotal quantities} 
\label{subsec: additive errors}
The additive errors framework exploits~\eqref{eq: regression error} by assuming that data are generated by
\begin{equation} \label{eq: additive errors}
    Y = f (\boldsymbol{x}) + \epsilon,
\end{equation}
where $\epsilon \sim P_{\epsilon}$ are zero-mean, $\mathrm{var} (\epsilon) = \sigma_{\epsilon}^2 < +\infty$, and $f$ has a finite $L_2$-norm, i.e., $\int f^2 (\boldsymbol{x}) d P_{\bx} < +\infty$, $P_{\bx}$ is an unspecified distribution for the predictors, e.g., uniform over an unknown manifold, and the errors are independent of $\boldsymbol{X}$. In this case, the training and out-of-sample data are iid realisations coming from~\eqref{eq: additive errors}, where the error distribution does not depend on $f (\boldsymbol{x})$. We say that these are {\em homoscedastic} errors. Prediction intervals can be derived by obtaining pivotal quantities as done by~\cite{pivot}. We assume that the parametric family the error distribution belongs to is known (e.g., a zero-mean normal distribution with unknown variance), select a fitting procedure and specify a regression family, and use analytical methods for obtaining a known sampling distribution for the prediction error. For example, if we assume that the data are generated by the simple linear regression $Y = \beta_0 + \beta_1 x + \epsilon$, where $\epsilon \sim \mathcal{N} (0, \sigma_{\epsilon}^2)$, and estimate the unknown parameters by least-squares, i.e., $\hat{f}_{\ell r} (x_o) = \hat{\beta}_0 + \hat{\beta}_1 \, x_o$. Then, for $\hat{\sigma}_{\epsilon}^2 = 1 / (\ntrain - 2) \, \sum_{i = 1}^{\ntrain}  ( y_i -  \hat{f}_{\ell r} (x_i) )^2$ and $\hat{\epsilon}_o = Y_o - \hat{f}_{\ell r} (x_o)$ we have that
\begin{equation} \label{eq: classic prediction interval}
    \hat{\epsilon}_o \, \left \{ (\ntrain - 2) \, \hat{\sigma}_{\epsilon}^2 \ \left ( 1 + \frac{1}{ n_{\mathrm{train}} } + \frac{(x_o - \overline{x}_{\mathrm{train}})^2 }{ \sum_{i = 1}^{n_{\mathrm{train}}} (x_i - \overline{x}_{\ntrain})^2  } \right) \right \}^{ - 1 / 2}
    \sim t (\ntrain - 2),
\end{equation}
where $t(\ntrain -2)$ is Student's $t$-distribution with $(\ntrain - 2)$ degrees of freedom; see, e.g.,~\cite{linear_models_book}.
%, i.e., the training set mean-squared prediction error 
The standardised prediction error, i.e., the left-hand side in~\eqref{eq: classic prediction interval} is an important and well-known pivotal quantity (its distribution does not depend on unknown parameters). The prediction intervals $ \widehat{C}_{\ell r} (x_o) $ are
\begin{equation} \label{eq: classic lin reg interval}
     \hat{f}_{\ell r} (x_o) \pm \left \{ (\ntrain - 2) \, \hat{\sigma}_{\epsilon}^2 \ \left ( 1 + \frac{1}{ n_{\mathrm{train}} } + \frac{(x_o - \overline{x}_{\mathrm{train}})^2 }{ \sum_{i = 1}^{n_{\mathrm{train}}} (x_i - \overline{x}_{\ntrain})^2  } \right) \right \}^{1 / 2} t_{ (\ntrain - 2), 1 - \alpha / 2} ,
\end{equation}
where $t_{ (\ntrain - 2), \, 1 - \alpha / 2} $ is the $(1 - \alpha / 2)$-quantile of $t (\ntrain -2)$. If these modelling assumptions are valid, then the interval in \eqref{eq: classic lin reg interval} is a confidence interval for $y_o$ at the $(1 - \alpha) \times 100\%$, i.e., for all $x_o$ it has valid conditional coverage,
$\prob (  Y_o \in \widehat{C}_{\ell r} (x_o) \, | \, X_o = x_o ) = 1 - \alpha . $
\par
Note that $\hat{f}_{\ell r} (x_o)$ is a consistent estimator of $\beta_0 + \beta_1 x_o$, and since Student's $t$-distribution converges to a standard normal as $n_{\mathrm{train}} \to +\infty$. In view of Lemma~\ref{lem: oracle and ideal coverage}, we see that $\widehat{C}_{\ell r} (x_o)$ is longer and converges in probability to the ideal interval for simple linear regression,
\begin{equation*}
    (\beta_0 + \beta_1 \, x_o ) \pm \sigma_{\epsilon} \, z_{1 - \alpha / 2},
\end{equation*}
where $z_{1 - \alpha / 2}$ is the $(1 - \alpha/ 2)$-quantile of the standard normal distribution, note that $ | z_{1 - \alpha / 2} | <  | t_{ (\ntrain - 2), \, 1 - \alpha / 2} |$. We remark that deriving closed-form prediction intervals without imposing assumptions on $f$ and $P_{\epsilon}$ can be challenging. Alternatively, we can use computational techniques, e.g., cross-validation~\citep{stone_cv} for estimating the generalisation error and its distribution. Simply put, to compute a valid model-agnostic prediction interval, we must estimate the prediction residual distribution.
%length of the interval depends on how much the out-of-sample observation deviates from the training set mean, i.e., $(x_o - \overline{x}_{\mathrm{train}})^2$. Further, more accurate predictions produce tighter prediction intervals (smaller $\hat{\sigma}_{\epsilon}^2$). 
%Our objective is estimating the distribution of $\hat{\epsilon}$ for any model $\hat{f}$, i.e., we do not assume anything about $f$. 

%We enlist three settings for computing prediction intervals by increasing complexity below.
%\begin{itemize}
%    \item Perhaps the most stringent setting is the classic one, i.e., $\epsilon \sim \mathcal{N}(0, \sigma_{\epsilon}^2)$. This setting can be extended to other known error distributions, e.g., $\epsilon \sim \mathrm{Laplace} (0, b)$. We refer to it as homoscedastic additive errors with known distribution. 
%    \item A useful relaxation is working with heteroscedastic additive errors, i.e., the error variance depends on $\boldsymbol{x}$, but the error distribution is specified, e.g., $\epsilon \sim \mathcal{N}(0, \sigma_{\epsilon}^2 (\boldsymbol{x}))$. We refer to it as heteroscedastic additive errors with known distribution. 
%    \item Estimating the prediction error distribution with nonparametric methods, i.e., $P_{\epsilon}$ is not specified. We refer to it as nonparametric additive errors, which can be homoscedastic or heterosdastic.
%\end{itemize}
%We propose prediction intervals for each of these in Sections~\ref{sec: lpm} and~\ref{sec: maps}.



==> jmlr-style-file-master/supplementary_material/theorem_one_proof.tex <==
\subsection{LPM with noise in the classic setting}
In the classic setting we assume that the LPM is given by
\begin{equation} \label{eq: classic setting lpm}
    \calb{Y} = y_{\beta} (\calb{\bx}) + u, 
\end{equation}
where $y_{\beta} (\calb{\bx}) := \beta_0 + \beta_1 \hat{f} (\calb{\bx})$, 
%$\var ( \calb{Y} ) = \var(f) + \sigma_{\epsilon}^2$, $\var(f) = \int \{f(\bx) - \mu(f) \}^2 dP_{\bx}$, $\mu(f) := \int f(\bx) dP_{\bx}$,
and the error linked to $\hat{f}$ is Gaussian, i.e., $u \sim \mathcal{N} (0, \sigma_{u}^2)$; see~\cite{salnikov2024liftedcoefficientdeterminationfast} for an earlier version of~\eqref{eq: classic setting lpm}. 
% \begin{remark}
    % The {\em LPM} given by~\eqref{eq: classic setting lpm} can be derived from a bivariate Gaussian assumption that links the correlation between calibration observations and model predictions;
%     Formally, it is derived from the conditional mean of $\calb{Y} \, | \, \hat{f} (\calb{\bx})$ if we assume that
%     \begin{equation*}
%     \begin{Bmatrix} 
%     \calb{Y} \\ \hat{f} (\calb{\bx}) 
%     \end{Bmatrix} \sim \mathcal{N}_2 \bigg [ \begin{Bmatrix} f(\calb{\bx}) \\ \overline{f} (\calb{\bx}) \end{Bmatrix},
%     \begin{pmatrix} \mathrm{var} (\calb{Y}) & \mathrm{cov} \{ \calb{Y}, \overline{f} (\calb{\bx}) \} \\ \mathrm{cov} \{ \calb{Y}, \overline{f} (\calb{\bx}) \} & \mathrm{var} (\overline{f}) \end{pmatrix} \bigg ].
% \end{equation*}
% \end{remark}
Note that~\eqref{eq: classic setting lpm} connects data generated by~\eqref{eq: regression error} with model predictions $\hat{f} (\calb{\bx})$ via a known joint distribution function. We stress that the random errors in~\eqref{eq: classic setting lpm} are {\em different} from the ones in~\eqref{eq: regression error}, i.e., $P_{u}$ is not the same as $P_{\epsilon}$, e.g., if~\eqref{eq: classic setting lpm} is valid, then $\var (u) = ( 1 - \rho^2) \{\var(f) + \sigma_{\epsilon}^2 \}$, which is equal to $\sigma_{\epsilon}^2$ if the regression function is constant, $f \equiv C$, or if $\beta_0 = 0$, $\beta_1 = 1$ and $\hat{f} \equiv f$ (in probability). Hence, we can derive a known prediction error distribution within the classic setting of linear regression with Gaussian errors. We estimate the unknown bias, $\beta_0$, and precision, $\beta_1$, coefficients in~\eqref{eq: classic setting lpm} by least-squares, and express the estimators in an alternative form, which highlights the interval's dependence on the correlation between model predictions and calibration response values.
The prediction interval, $\widehat{C}_{\ell pm} (\bx_o)$, is 
\begin{equation} \label{eq: b0 lpm prediction interval}
     \hat{y}_{\beta} (\bx_o) \pm \left \{ \left [1 + 1 / (n_{\mathrm{cal}} - 2) \right ] \left [ 1 - \calb{R^2} (\hat{f}) \right ] s_{\calb{\boldsymbol{y}}}^2 \left [ 1 + \widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) \right ] \right \}^{ 1 / 2 } t_{(n_{\mathrm{cal}} - 2), 1 - \alpha / 2},
\end{equation}
where $\hat{y}_{\beta} (\bx_o) := \hat{\beta}_0 + \hat{\beta}_1 \, \hat{f} (\x_o )$ are lifted predictions, $ \overline{\mu}_{\hat{f}} := ( 1 / \calb{n}) \, \sum_{\calb{i} = 1}^{\calb{n}} \hat{f} (\bx_{\calb{i}})$,
$$\widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) := \frac{1}{ n_{\mathrm{cal}} } + \frac{( \hat{f} (\bx_o) - \overline{\mu}_{\hat{f}})^2 }{ \sum_{i = 1}^{n_{\mathrm{cal}}} ( \hat{f} ( \bx_{\calb{i}}) -  \overline{\mu}_{\hat{f}})^2  }, $$
%% \begin{align*}
%     &\overline{y}_{\mathrm{cal}} = 1 / n_{\mathrm{cal}}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} y_{i_{\mathrm{cal}}}, \, \, \, \, \, \, \, \, \, \, \, \,  s_{y_{\mathrm{cal}}}^2 = (n_{\mathrm{cal}} - 1)^{-1}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} (y_{i_{\mathrm{cal}}} - \overline{y}_{\mathrm{cal}} )^2, \\
%     &\hat{\mu}_{\mathrm{cal}} = 1 / n_{\mathrm{cal}}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} \hat{f} (\boldsymbol{x}_{i_{\mathrm{cal}}}), \, \, \, \, \, \,
%     s_{\hat{f}}^2 = (n_{\mathrm{cal}} - 1)^{-1}  \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} \{ \hat{f} (\boldsymbol{x}_{i_{\mathrm{cal}}}) - \hat{\mu}_{\mathrm{cal}} \}^2,
% \end{align*}
% are sample mean and standard deviation statistics for response and model predictions in the calibration set, and
and $\calb{R} (\hat{f})$
    %$= \left [ \sum_{i_{\mathrm{cal}} = 1}^{n_{\mathrm{cal}}} (y_{i_{\mathrm{cal}}} - \overline{y}_{\mathrm{cal}})  \{ \hat{f} (\boldsymbol{x}_{i_{\mathrm{cal}}}) - \hat{\mu}_{\mathrm{cal}} \} \right ] / ( s_{y_{\mathrm{cal}}} \, s_{\hat{f}} )$
is the correlation coefficient between $\calb{\boldsymbol{y}}$ and $\{ \hat{f} (\boldsymbol{x}_{1_{\mathrm{cal}}}), \dots, \hat{f} (\boldsymbol{x}_{n_{\mathrm{cal}}}) \}$.
\par
The prediction interval $\widehat{C}_{\ell pm} (\bx_o)$ is model-agnostic at the $(1 - \alpha) \times 100\%$ confidence level, i.e., it is a valid non-trivial prediction interval for any model $\hat{f}$. Further, it suggests comparing predictive models using correlation values, since its length {\em decreases} the closer $R_{\mathrm{cal}}^2 (\hat{f})$ is to one, and that the MSPE of lifted predictions is smaller than the one of model predictions $\hat{f} (\calb{\bx})$.
%, i.e., $\sum_{\calb{i} = 1}^{\calb{n}} (y_{\calb{i}} - \hat{y}_{\beta} (\bx_{\calb{i}}) )^2 \leq \sum_{\calb{i} = 1}^{\calb{n}} (y_{\calb{i}} - \hat{f} (\bx_{\calb{i}}) )^2$. 
Theorem~\ref{th: t student interval} makes these statements precise.
\begin{theorem} \label{th: t student interval}
    Assume that~\eqref{eq: classic setting lpm} is valid. Then, given $\hat{f} (\boldsymbol{x}_o)$ and $\{ \hat{f} (\boldsymbol{x}_{1_{\mathrm{cal}}}), \dots, \hat{f} (\boldsymbol{x}_{n_{\mathrm{cal}}}) \}$, for all $\alpha \in (0, 1)$ we have that
    % \begin{equation} \label{eq: t-student distribution}
    %     U_o / \big \{ a^2 \big(1 - R^2_{\mathrm{cal}} (\hat{f}) \big) s_{y_{\mathrm{cal}}}^2 \hat{\eta} (\boldsymbol{x}_o ) \big \}^{ 1 / 2 } \sim t (n_{\mathrm{cal}} - 2),
    % \end{equation}
    % where $t (n_{\mathrm{cal}} - 2)$ is Student's t-distribution with $(n_{\mathrm{cal}} - 2)$ degrees of freedom. Thus, for $\alpha \in (0, 1)$ we have that
            \begin{equation} \label{eq: point estimator concentration}
                  \mathbf{Pr} \big ( Y_o \in \widehat{C}_{\ell pm} (\bx_o) \, | \, \bX_o = \bx_o \big ) = 1 - \alpha.
            \end{equation}
    Further, for homoscedastic errors, not necessarily Gaussian, the {\em MSPE} can be bounded as
    \begin{equation}
        \operatorname{MSPE} [ f (\bx_o)] \leq \operatorname{MSPE} [y_{\beta} (\bx_o)] \leq \operatorname{MSPE} [\hat{f} (\bx_o)],
    \end{equation}
    and we have that
    \begin{equation*}
        \operatorname{MSPE} [\hat{y}_{\beta} (\bx_o)] = \operatorname{MSPE} [y_{\beta} (\bx_o)] + o( 1 / \, \calb{n}).
    \end{equation*}
    % \begin{multline} \label{eq: mspe lower bound}
    %         \sigma_{\epsilon}^2 + \sigma_u^2 \mathbb{E} \big[ \widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) \big] \leq \operatorname{MSPE} [\hat{y}_{\beta} (\bx_o)]
    %         \leq \sigma_{\epsilon}^2 + \sigma_u^2 \mathbb{E} \big[ \widehat{\eta}_{\hat{f}} ( \boldsymbol{x}_o ) \big] \\
    %        + 2 \left ( \beta_1^2 \, \operatorname{MSPE} [\hat{f} (\bx_o)] + \{ \beta_0 + (\beta_1 - 1) f (\bx_o) \}^2 \right ).
    % \end{multline}
\end{theorem}
\par
Theorem~\ref{th: t student interval} allows us to compute fast model-agnostic conditional prediction intervals with valid finite sample coverage, albeit in the classic setting~\eqref{eq: classic setting lpm}. To the best of our knowledge, there are no other closed-form solution prediction intervals with these properties. Further, if $\hat{f}$ is consistent ($\| \hat{f} - f \|_{\infty} = o_{\mathbf{Pr}} (1)$), then $\hat{y}_{\beta}$ is also consistent, $| \hat{y}_{\beta} (\bx_o) - \hat{f} (\bx_o) | = o_{\mathbf{Pr}} (1)$ and $\widehat{C}_{\ell pm} (\bx_o)$ converges in probability to $C_{\mathrm{ideal}} (\bx_o)$. MAPS generalises $\widehat{C}_{\ell pm} (\bx_o)$ to the distribution-free setting.

